Trust Implications of DDoS Protection in Online Elections

Online elections make a natural target for distributed denial of service attacks. Election agencies wary of disruptions to voting may procure DDoS protection services from a cloud provider. However, current DDoS detection and mitigation methods come at the cost of significantly increased trust in the cloud provider. In this paper we examine the security implications of denial-of-service prevention in the context of the 2017 state election in Western Australia, revealing a complex interaction between actors and infrastructure extending far beyond its borders. Based on the publicly observable properties of this deployment, we outline several attack scenarios including one that could allow a nation state to acquire the credentials necessary to man-in-the-middle a foreign election in the context of an unrelated domestic law enforcement or national security operation, and we argue that a fundamental tension currently exists between trust and availability in online elections.

==> subjidx.tex <==
%                                                           clmomu01.ind
%-----------------------------------------------------------------------
% CLMoMu01 1.0: LaTeX style files for books
% Sample index file for User's guide
% (c) Springer-Verlag HD
%-----------------------------------------------------------------------
\begin{theindex}
\item Absorption\idxquad 327
\item Absorption of radiation \idxquad 289--292,\, 299,\,300
\item Actinides \idxquad 244
\item Aharonov-Bohm effect\idxquad 142--146
\item Angular momentum\idxquad 101--112
\subitem algebraic treatment\idxquad 391--396
\item Angular momentum addition\idxquad 185--193
\item Angular momentum commutation relations\idxquad 101
\item Angular momentum quantization\idxquad 9--10,\,104--106
\item Angular momentum states\idxquad 107,\,321,\,391--396
\item Antiquark\idxquad 83
\item $\alpha$-rays\idxquad 101--103
\item Atomic theory\idxquad 8--10,\,219--249,\,327
\item Average value\newline ({\it see also\/} Expectation value)
15--16,\,25,\,34,\,37,\,357
\indexspace
\item Baker-Hausdorff formula\idxquad 23
\item Balmer formula\idxquad 8
\item Balmer series\idxquad 125
\item Baryon\idxquad 220,\,224
\item Basis\idxquad 98
\item Basis system\idxquad 164,\,376
\item Bell inequality\idxquad 379--381,\,382
\item Bessel functions\idxquad 201,\,313,\,337
\subitem spherical\idxquad 304--306,\, 309,\, 313--314,\,322
\item Bound state\idxquad 73--74,\,78--79,\,116--118,\,202,\, 267,\,
273,\,306,\,348,\,351
\item Boundary conditions\idxquad 59,\, 70
\item Bra\idxquad 159
\item Breit-Wigner formula\idxquad 80,\,84,\,332
\item Brillouin-Wigner perturbation theory\idxquad 203
\indexspace
\item Cathode rays\idxquad 8
\item Causality\idxquad 357--359
\item Center-of-mass frame\idxquad 232,\,274,\,338
\item Central potential\idxquad 113--135,\,303--314
\item Centrifugal potential\idxquad 115--116,\,323
\item Characteristic function\idxquad 33
\item Clebsch-Gordan coefficients\idxquad 191--193
\item Cold emission\idxquad 88
\item Combination principle, Ritz's\idxquad 124
\item Commutation relations\idxquad 27,\,44,\,353,\,391
\item Commutator\idxquad 21--22,\,27,\,44,\,344
\item Compatibility of measurements\idxquad 99
\item Complete orthonormal set\idxquad 31,\,40,\,160,\,360
\item Complete orthonormal system, {\it see}\newline
Complete orthonormal set
\item Complete set of observables, {\it see\/} Complete
set of operators
\indexspace
\item Eigenfunction\idxquad 34,\,46,\,344--346
\subitem radial\idxquad 321
\subsubitem calculation\idxquad 322--324
\item EPR argument\idxquad 377--378
\item Exchange term\idxquad 228,\,231,\,237,\,241,\,268,\,272
\indexspace
\item $f$-sum rule\idxquad 302
\item Fermi energy\idxquad 223
\indexspace
\item H$^+_2$ molecule\idxquad 26
\item Half-life\idxquad 65
\item Holzwarth energies\idxquad 68
\end{theindex}

